Revisiting Prefix-tuning: Statistical Benefits of Reparameterization among Prompts

Prompt-based techniques, such as prompt-tuning and prefix-tuning, have gained prominence for their efficiency in fine-tuning large pre-trained models. Despite their widespread adoption, the theoretical foundations of these methods remain limited. For instance, in prefix-tuning, we observe that a key factor in achieving performance parity with full fine-tuning lies in the reparameterization strategy. However, the theoretical principles underpinning the effectiveness of this approach have yet to be thoroughly examined. Our study demonstrates that reparameterization is not merely an engineering trick but is grounded in deep theoretical foundations. Specifically, we show that the reparameterization strategy implicitly encodes a shared structure between prefix key and value vectors. Building on recent insights into the connection between prefix-tuning and mixture of experts models, we further illustrate that this shared structure significantly improves sample efficiency in parameter estimation compared to non-shared alternatives. The effectiveness of prefix-tuning across diverse tasks is empirically confirmed to be enhanced by the shared structure, through extensive experiments in both visual and language domains. Additionally, we uncover similar structural benefits in prompt-tuning, offering new perspectives on its success. Our findings provide theoretical and empirical contributions, advancing the understanding of prompt-based methods and their underlying mechanisms.

==> arxiv/datasets.tex <==
\begin{table}[t]
\caption{Specifications of datasets evaluated for visual tasks. Following \cite{jia2022visual}, we randomly sampled the train and val sets since there are no public splits available.}
\label{table:datasets}
\begin{center}
\scalebox{0.75}{
\begin{tabular}{@{}llllll@{}}
\toprule
\textbf{Dataset} & \textbf{Description}                         & \textbf{\# Classes} & \textbf{Train}            & \textbf{Val}         & \textbf{Test} \\ \midrule
\textit{Fine-grained visual recognition tasks (FGVC)}    &       &                &                    &                 &          \\ \cmidrule(l){2-6} 
CUB-200-2011 \cite{wah2011caltech}    & Fine-grained bird species recognition        & 200                 & 5,394                     & 600                  & 5,794         \\
NABirds \cite{van2015building}         & Fine-grained bird species recognition        & 55                  & 21,536                    & 2,393                & 24,633        \\
Oxford Flowers \cite{nilsback2008automated}  & Fine-grained flower species recognition      & 102                 & 1,020                     & 1,020                & 6,149         \\
Stanford Dogs \cite{khosla2011novel}   & Fine-grained dog species recognition         & 120                 & 10,800                    & 1,200                & 8,580        \\
Stanford Cars \cite{gebru2017fine}   & Fine-grained car recognition                 & 196                 & 7,329                     & 815                  & 8,041         \\ \midrule
\textit{Visual Task Adaptation Benchmark (VTAB-1K)}    &       &                &                    &                 &          \\ \cmidrule(l){2-6}                     
CIFAR-100 \cite{Krizhevsky09learningmultiple}       & \multicolumn{1}{l}{\multirow{7}{*}{Natural}} & 100                 & \multirow{7}{*}{800/1000} & \multirow{7}{*}{200} & 10,000              \\
Caltech101 \cite{fei2006one} & \multicolumn{1}{c}{}                         &  102          &                           &                      &  6,084            \\
DTD \cite{cimpoi2014describing} & \multicolumn{1}{c}{}                         &  47          &                           &                      &  1,880            \\
Flowers102 \cite{nilsback2008automated} & \multicolumn{1}{c}{}                         &  102          &                           &                      &  6,149            \\
Pets \cite{parkhi2012cats} & \multicolumn{1}{c}{}                         &  37          &                           &                      &  3,669            \\
SVHN \cite{netzer2011reading} & \multicolumn{1}{c}{}                         &  10          &                           &                      &  26,032            \\
Sun397 \cite{xiao2010sun}          & \multicolumn{1}{c}{}                         & 397                 &                           &                      &   21,750           \\ \cmidrule(l){2-6} 
Patch Camelyon \cite{veeling2018rotation} & \multirow{4}{*}{Specialized}                 &    2     & \multirow{4}{*}{800/1000}         & \multirow{4}{*}{200}    & 32,768              \\
EuroSAT  \cite{helber2019eurosat}   &                 &    10    &                           &                      &  5,400    \\
Resisc45 \cite{cheng2017remote}   &            &       45         &                           &                      &   6,300            \\
Retinopathy \cite{graham2015kaggle} &             &   5       &                           &                      &   42,670      \\ \cmidrule(l){2-6} 
Clevr/count \cite{johnson2017clevr} & \multirow{8}{*}{Structured}                  &   8        & \multirow{8}{*}{800/1000}         & \multirow{8}{*}{200}    & 15,000   \\
Clevr/distance \cite{johnson2017clevr}   &       &    6      &         &              &  15,000             \\
DMLab \cite{beattie2016deepmind}  &         &     6     &      &          &    22,735  \\
KITTI/distance \cite{geiger2013vision}  &         &    4     &         &             &   711   \\
dSprites/loc \cite{matthey2017dsprites}  &       &   16  &         &              &   73,728           \\
dSprites/ori \cite{matthey2017dsprites} &       &    16    &        &        &  73,728     \\
SmallNORB/azi \cite{lecun2004learning}  &           &   18     &                 &                      &    12,150  \\
SmallNORB/ele \cite{lecun2004learning}  &           &   9    &       &               &   12,150   \\ \bottomrule
\end{tabular}
}
\end{center}
\end{table}



==> arxiv/fgvc_per_task.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\caption{Per-task fine-tuning results for FGVC benchmarks. We report the average accuracy over five independent runs. Best results among all methods are \textbf{bolded}.}
\label{table:fgvc}
\begin{center}
\scalebox{0.82}{
\begin{tabular}{@{}l|cccccc@{}}
\toprule
\multicolumn{1}{c|}{\textbf{Method}} & \textbf{CUB-200-2011} & \textbf{NABirds} & \textbf{Oxford Flowers} & \textbf{Stanford Dogs} & \textbf{Stanford Cars} & \textbf{Mean Acc} \\ \midrule
Deep-$\mathrm{share}_{\texttt{SHALLOW}}$                         & 87.2                  & 81.5             & 98.6                    & 91.1                   & 63.4                   & 84.36             \\
Simple-$\mathrm{share}_{\texttt{SHALLOW}}$                      & 86.6                  & 79.3             & 98.4                    & 90.8                   & 55.4                   & 82.10              \\
No-$\mathrm{share}_{\texttt{SHALLOW}}$                            & 85.1                  & 77.8             & 97.9                    & 86.4                   & 54.7                   & 80.38             \\
Deep-$\mathrm{share}_{\texttt{DEEP}}$                          & 87.8                  & \textbf{84.5}    & 98.2                    & \textbf{91.6}          & 79.3                   & 88.28             \\
Simple-$\mathrm{share}_{\texttt{DEEP}}$                          & \textbf{88.7}         & 84.3             & \textbf{98.8}           & 90.6                   & \textbf{82.8}          & \textbf{89.04}    \\
No-$\mathrm{share}_{\texttt{DEEP}}$                               & 85.9                  & 79.0             & 97.9                    & 86.3                   & 62.5                   & 82.32             \\ \bottomrule
\end{tabular}}
\end{center}
\end{table}

==> arxiv/macro_commands.tex <==
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

% Parameter Estimation

\newcommand{\dbzijn}{\Delta \beta_{0ij}^{n}}
\newcommand{\dboijn}{\Delta \beta_{1ij}^{n}}
\newcommand{\daijn}{\Delta a_{ij}^{n}}
\newcommand{\dbijn}{\Delta b_{ij}^{n}}
\newcommand{\dsijn}{\Delta \sigma_{ij}^{n}}
%\newcommand{\norm}[1]{\|#1\|}

\newcommand{\bzin}{\beta^{n}_{0i}}
\newcommand{\boin}{\beta^{n}_{1i}}
\newcommand{\ain}{a_i^n}
\newcommand{\bin}{b_i^n}
\newcommand{\sigmain}{\sigma_i^n}

\newcommand{\bzj}{\beta_{0j}^{*}}
\newcommand{\boj}{\beta_{1j}^{*}}
\newcommand{\aj}{a_{j}^{*}}
\newcommand{\bj}{b_{j}^{*}}
\newcommand{\sigmaj}{\sigma_{j}^{*}}

\newcommand{\bzjp}{\beta_{0j'}^{*}}
\newcommand{\bojp}{\beta_{1j'}^{*}}
\newcommand{\ajp}{a_{j'}^{*}}
\newcommand{\bjp}{b_{j'}^{*}}
\newcommand{\sigmajp}{\sigma_{j'}^{*}}

\newcommand{\zerod}{\mathbf{0}_d}
\newcommand{\ktilde}{\tilde{k}}
\newcommand{\Dtilde}{\widetilde{D}}

\newcommand{\brj}{\bar{r}(|\mathcal{A}_j|)}
\newcommand{\trj}{\tilde{r}(|\mathcal{A}_j|)}
\newcommand{\trjp}{\tilde{r}(|\mathcal{A}_{j'}|)}

%%% j* = 1
\newcommand{\brone}{\bar{r}(|\mathcal{A}_1|)}
\newcommand{\dboione}{\Delta_{t_2} \beta_{1i1}^{n}}
\newcommand{\dbzione}{\Delta \beta_{0i1}^{n}}
\newcommand{\daione}{\Delta a_{i1}^{n}}
\newcommand{\dbione}{\Delta b_{i1}^{n}}
\newcommand{\dsione}{\Delta \sigma_{i1}^{n}}

\newcommand{\trone}{\tilde{r}(|\mathcal{A}_1|)}
\newcommand{\trs}{\tilde{r}(|\mathcal{A}_{j^*}|)}

\newcommand{\dint}{\mathrm{d}}


\newcommand{\brackets}[1]{\left[ #1 \right]}
\newcommand{\parenth}[1]{\left( #1 \right)}
\newcommand{\bigparenth}[1]{\big( #1 \big)}
\newcommand{\biggparenth}[1]{\bigg( #1 \bigg)}
\newcommand{\braces}[1]{\left\{ #1 \right \}}
\newcommand{\abss}[1]{\left| #1 \right |}
\newcommand{\angles}[1]{\left\langle #1 \right \rangle}
\newcommand{\tp}{^\top}
% \newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\def\argmin{\textnormal{arg} \min}
\def\st{\textnormal{s.t.}}
\def\sgn{\texttt{sign}}
% \newcommand{\todo}[1]{\textcolor{red}{[Todo: #1]}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

\def\TM{\texttt{T}}
\def\OT{\textnormal{OT}}
\def\TW{\textnormal{TW}}
\def\TSW{\textnormal{TSW}}


\def\RR{\mathbb{R}}
\def\DD{\mathbb{D}}
\def\NN{\mathbb{N}}
\def\PP{\mathbb{P}}
\def\MM{\mathbb{M}}
\def\SS{\mathbb{S}}
\def\EE{\mathbb{E}}
\def\FF{\mathbb{F}}
\def\TT{\mathbb{T}}
\def\XX{\mathbb{X}}
\def\QQ{\mathbb{Q}}
\def\FF{\mathbb{F}}

\def\Ff{\mathcal{F}}
\def\Hh{\mathcal{H}}
\def\Gg{\mathcal{G}}
\def\Ee{\mathcal{E}}
\def\Pp{\mathcal{P}}
\def\Ss{\mathcal{S}}
\def\Ww{\mathcal{W}}
\def\Ff{\mathcal{F}}
\def\Rr{\mathcal{R}}
\def\Nn{\mathcal{N}}
\def\Xx{\mathcal{X}}
\def\Tt{\mathcal{T}}
\def\Mm{\mathcal{M}}
\def\Qq{\mathcal{Q}}

\newcommand{\xbm}{{\bm x}}
\newcommand{\Xbm}{{\bm X}}

\newcommand{\ybm}{{\bm y}}
\newcommand{\Ybm}{{\bm Y}}

\newcommand{\pbm}{{\bm p}}
\newcommand{\Pbm}{{\bm P}}


\newcommand{\wbm}{{\bm w}}
\newcommand{\Wbm}{\bm{W}}
\newcommand{\Wq}{\Wbm^{\rm q}}
\newcommand{\Wk}{\Wbm^{\rm k}}
\newcommand{\Wv}{\Wbm^{\rm v}}

\newcommand{\bbm}{{\bm b}}
\newcommand{\bq}{\bbm^{\rm q}}
\newcommand{\bk}{\bbm^{\rm k}}

\newcommand{\Abm}{{\bm A}}
\newcommand{\cbm}{{\bm c}}


\newcommand{\kbm}{{\bm k}}
\newcommand{\Kbm}{{\bm K}}

\newcommand{\ubm}{{\bm u}}
\newcommand{\Ubm}{{\bm U}}

\newcommand{\vbm}{{\bm v}}
\newcommand{\Vbm}{{\bm V}}

\newcommand{\qbm}{{\bm q}}
\newcommand{\Qbm}{{\bm Q}}

\newcommand{\abm}{{\bm \alpha}}
\newcommand{\sbm}{{\bm s}}
\newcommand{\gbm}{{\bm g}}
\newcommand{\hbm}{{\bm h}}

\newcommand{\ebm}{{\bm e}}
\newcommand{\zbm}{{\bm z}}



% \newcommand{\vtheta}{{\bm \theta}}
\newcommand{\veta}{{\bm \eta}}


\newcommand{\LS}{\mathcal{LS}}
\newcommand{\NS}{\mathcal{NS}}
\newcommand{\CS}{\mathcal{CS}}
\newcommand{\NCS}{\mathcal{NCS}}
\newcommand{\CSb}{\mathcal{CS}\text{-b}}
\newcommand{\CSd}{\mathcal{CS}\text{-d}}
\newcommand{\CSs}{\mathcal{CS}\text{-s}}
\newcommand{\NCSb}{\mathcal{NCS}\text{-b}}
\newcommand{\NCSd}{\mathcal{NCS}\text{-d}}
\newcommand{\NCSs}{\mathcal{NCS}\text{-s}}
\newcommand{\CSW}{\text{CSW}}
\newcommand{\NCSW}{\text{NCSW}}
\newcommand{\NCSWb}{\mathcal{NCSW}\text{-b}}
\newcommand{\NCSWd}{\mathcal{NCSW}\text{-d}}
\newcommand{\NCSWs}{\mathcal{NCSW}\text{-s}}

\newcommand{\pop}{F}
\newcommand{\nop}{F_n}
\newcommand{\popNGD}{F^{\texttt{NGD}}}
\newcommand{\nopNGD}{F_n^{\texttt{NGD}}}

\newcommand{\xbf}{\mathbf{x}}
\newcommand{\ybf}{\mathbf{y}}
\newcommand{\wbf}{\mathbf{w}}
\newcommand{\bbf}{\mathbf{b}}

\newcommand*{\vertbar}{\rule[-1ex]{0.5pt}{2.5ex}}
\newcommand*{\horzbar}{\rule[.5ex]{2.5ex}{0.5pt}}

\newcommand{\NormGD}{NormGD}
\newcommand{\ds}{\displaystyle}



% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
%---------------------------
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\var}{\mathrm{Var}}


\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\mathrm{sigmoid}}
\newcommand{\gelu}{\mathrm{GELU}}
% \newcommand{\tanh}{\mathrm{tanh}}



% Some abbreviations
\def\st{{\em s.t.~}}
\def\ie{{\em i.e.,~}}
\def\eg{{\em e.g.,~}}
\def\cf{{\em cf.,~}}
\def\ea{{\em et al.~}}
\newcommand{\iid}{i.i.d.}
\newcommand{\wrt}{w.r.t.}


\newcommand{\deijn}{\Delta \eta_{ij}^{n}}

\newcommand{\dboin}{\Delta \beta_{1i}^{n}}
\newcommand{\dbzin}{\Delta \beta_{0i}^{n}}

\newcommand{\dain}{\Delta a_{i}^{n}}
\newcommand{\dbin}{\Delta b_{i}^{n}}
\newcommand{\dein}{\Delta \eta_{i}^{n}}


\newcommand{\cin}{c_i^n}
\newcommand{\ein}{\eta_i^n}

\newcommand{\boonen}{\beta_{11}^n}
\newcommand{\bzonen}{\beta_{01}^n}
\newcommand{\aonen}{a_1^n}
\newcommand{\bonen}{b_1^n}
\newcommand{\eonen}{\eta_1^n}

%\newcommand{\boj}{\beta_{1j}^*}
\newcommand{\coj}{c_j^0}
\newcommand{\coi}{c_i^0}

\newcommand{\aaoj}{A_j^0}
\newcommand{\aaoi}{A_i^0}

\newcommand{\eoj}{\eta_j^0}
\newcommand{\eoi}{\eta_i^0}

\newcommand{\cj}{c_j^*}

\newcommand{\ej}{\eta_j^*}

\newcommand{\boi}{\beta_{1i}^*}
\newcommand{\bzi}{\beta_{0i}^*}
\newcommand{\ai}{a_i^*}
\newcommand{\bi}{b_i^*}
\newcommand{\ei}{\eta_i^*}

\newcommand{\boone}{\beta_{11}^*}
\newcommand{\bzone}{\beta_{01}^*}
\newcommand{\aone}{a_1^*}
\newcommand{\bone}{b_1^*}
\newcommand{\eone}{\eta_1^*}

\newcommand{\cjp}{c_{j'}^0}
\newcommand{\gjp}{\Gamma_{j'}^0}
\newcommand{\ejp}{\eta_{j'}^0}


\newcommand{\zeroq}{\mathbf{0}_q}
\newcommand{\pizeroone}{\pi_{1}^{0}}
%\newcommand{\dboione}{\Delta \beta_{1i1}^{n}}
\newcommand{\dtone}{\Delta \tau^{n}}

\newcommand{\deione}{\Delta \eta_{i1}^{n}}



\newcommand{\normf}[1]{\|#1\|_{L^2(\mu)}}

\newcommand{\bfit}[1]{\boldsymbol{#1}}

\newcommand{\prompt}{\bm p}
\newcommand{\dt}{\mathcal{D}_t}
\newcommand{\data}{\mathcal{D}}

\newcommand{\xdom}{\mathcal{X}^{(t)}}
\newcommand{\ydom}{\mathcal{Y}^{(t)}}


\newcommand{\yi}{\mathcal{Y}^{(i)}}
\newcommand{\yj}{\mathcal{Y}^{(j)}}


\newcommand{\normop}{\mathcal{S}_p}
\newcommand{\att}{\mathrm{Attention}}
\newcommand{\dv}{d_v}
\newcommand{\dk}{d_k}

\def\mmoe{\texttt{MMoE}}


==> arxiv/metrics.tex <==
\begin{table}[t]
\caption{Evaluation metrics for each dataset.}
\label{table:metrics}
\begin{center}
\scalebox{1.0}{
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Datasets} & \textbf{Task}                     & \textbf{Metrics}                            \\ \midrule
FGVC     & Image classification     & Accuracy                           \\
VTAB-1K  & Image classification     & Accuracy                           \\
E2E      & Table-to-text generation & BLEU, NIST, METEOR, ROUGE-L, CIDEr \\
WebNLG   & Table-to-text generation & BLEU, METEOR, TER                  \\
XSUM     & Summarization            & ROUGE-1, ROUGE-2, ROUGE-L          \\ \bottomrule
\end{tabular}}
\end{center}
\end{table}

==> arxiv/peft_nlp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{Comparison of fine-tuning results between common techniques on E2E and WebNLG.}
\label{table:peft_nlp}
\begin{center}
\scalebox{0.825}{
\begin{tabular}{@{}l|ccccc|ccccccccc@{}}
\toprule
\multirow{3}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{E2E}} & \multicolumn{9}{c}{\textbf{WebNLG}}                                          \\
                                 & BLEU & NIST & MET  & R-L  & CIDEr & \multicolumn{3}{c}{BLEU} & \multicolumn{3}{c}{MET} & \multicolumn{3}{c}{TER $\downarrow$} \\
                                 &      &      &      &      &       & S      & U      & A      & S      & U      & A     & S      & U      & A     \\ \midrule
Finetune                         & 68.2 & 8.62 & 46.2 & 71.0 & 2.47  & 64.2   & 27.7   & 46.5   & 0.45   & 0.30   & 0.38  & 0.33   & 0.76   & 0.53  \\
Partial-2                        & 68.1 & 8.59 & 46.0 & 70.8 & 2.41  & 53.6   & 18.9   & 36.0   & 0.38   & 0.23   & 0.31  & 0.49   & 0.99   & 0.72  \\
Adapter                          & 66.3 & 8.41 & 45.0 & 69.8 & 2.40  & 54.5   & 45.1   & 50.2   & 0.39   & 0.36   & 0.38  & 0.40   & 0.46   & 0.43  \\ \midrule
No-share                         & 68.0 & 8.61 & 45.8 & 71.0 & 2.41  & 61.1   & 42.8   & 53.5   & 0.43   & 0.35   & 0.40  & 0.36   & 0.49   & 0.42  \\
Deep-share                       & 69.9 & 8.78 & 46.3 & 71.5 & 2.45  & 63.9   & 44.3   & 54.5   & 0.45   & 0.36   & 0.41  & 0.34   & 0.52   & 0.42  \\ \bottomrule
\end{tabular}}
\end{center}
\end{table}

==> arxiv/peft_vision.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{Comparison of fine-tuning results between common techniques on FGVC and VTAB-1K.}
\label{table:peft_cv}
\begin{center}
\scalebox{1.0}{
\begin{tabular}{@{}l|cccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multirow{2}{*}{\textbf{FGVC}} & \multicolumn{3}{c}{\textbf{VTAB-1K}} \\
\multicolumn{1}{c|}{}                                 &                                & Natural  & Specialized  & Structural \\ \midrule
Finetune                                              & 88.54                          & 75.88    & 83.36        & 47.64      \\
Partial-1                                             & 82.63                          & 69.44    & 78.53        & 34.17      \\
Adapter                                               & 85.66                          & 70.39    & 77.11        & 33.43      \\
VPT-Shallow                                           & 84.62                          & 76.81    & 79.66        & 46.98      \\
VPT-Deep                                              & 89.11                          & 78.48    & 82.43        & 54.98      \\ \midrule
No-$\mathrm{share}_{\texttt{SHALLOW}}$                                      & 80.38                          & 69.00    & 77.20        & 29.65      \\
No-$\mathrm{share}_{\texttt{DEEP}}$                                           & 82.32                          & 70.29    & 80.20        & 37.69      \\
Deep-$\mathrm{share}_{\texttt{SHALLOW}}$                                     & 84.36                          & 75.79    & 79.48        & 38.53      \\
Deep-$\mathrm{share}_{\texttt{DEEP}}$                                       & 88.28                          & 77.06    & 82.28        & 52.00      \\ \bottomrule
\end{tabular}}
\end{center}
\end{table}


==> arxiv/share_nonshare_nlp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{Comparison of prefix-tuning with and without reparameterization on language datasets including E2E, WebNLG, and XSUM. Best results among all methods except Finetune are \textbf{bolded}.} 
\label{table:shared_noshared_nlp}
\vspace{-0.5em}
\begin{center}
\scalebox{0.675}{
\begin{tabular}{@{}l|ccccc|ccccccccc|ccc@{}}
\toprule
\multirow{3}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{E2E}}          & \multicolumn{9}{c|}{\textbf{WebNLG}}                                                   & \multicolumn{3}{c}{\textbf{XSUM}} \\
                        & BLEU & NIST & MET  & R-L  & CIDEr & \multicolumn{3}{c}{BLEU} & \multicolumn{3}{c}{MET} & \multicolumn{3}{c|}{TER $\downarrow$} & R-1    & R-2    & R-L    \\
                        &      &      &      &      &       & S      & U      & A      & S      & U      & A     & S      & U      & A      &        &        &        \\ \midrule
Finetune                & 68.2 & 8.62 & 46.2 & 71.0 & 2.47  & 64.2   & 27.7   & 46.5   & 0.45   & 0.30   & 0.38  & 0.33   & 0.76   & 0.53   & 45.14  & 22.27  & 37.25  \\
Deep-share              & \textbf{69.9} & \textbf{8.78} & \textbf{46.3} & \textbf{71.5} & \textbf{2.45}  & \textbf{63.9}   & \textbf{44.3}   & \textbf{54.5}   & \textbf{0.45}   & \textbf{0.36}   & \textbf{0.41}  & \textbf{0.34}   & 0.52   & \textbf{0.42}   & \textbf{42.62}  & \textbf{19.66}  & \textbf{34.36}  \\
No-share                & 68.0 & 8.61 & 45.8 & 71.0 & 2.41  & 61.1   & 42.8  & 53.5  & 0.43   & 0.35   & 0.40  & 0.36   & \textbf{0.49}   & \textbf{0.42}   & 36.86  & 15.16  & 29.89  \\ \bottomrule
\end{tabular}}
\end{center}
\vspace{-1 em}
\end{table}


==> arxiv/share_nonshare_vision.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{Comparison of prefix-tuning with and without reparameterization on FGVC and VTAB-1K benchmarks. We report the average accuracy over five independent runs. Best results among all methods except Finetune are \textbf{bolded}.}
\label{table:shared_noshared_cv}
\vspace{-0.5em}
\begin{center}
\scalebox{0.645}{
\begin{tabular}{@{}l|cccccc|ccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{6}{c|}{\textbf{FGVC}}                                                          & \multicolumn{3}{c}{\textbf{VTAB-1K}}        \\
\multicolumn{1}{c|}{}                        & Mean Acc & CUB-200-2011 & NABirds & Oxford Flowers & Stanford Dogs & Stanford Cars & Natural & Specialized & Structured \\ \midrule
Finetune                                     & 88.54    & 87.3         & 82.7    & 98.8           & 89.4          & 84.5          & 75.88   & 83.36       & 47.64      \\
Deep-$\mathrm{share}_{\texttt{SHALLOW}}$                          & 84.36    & 87.2         & 81.5    & \textbf{98.6}           & 91.1          & 63.4          & 75.79   & 79.48       & 38.53      \\
No-$\mathrm{share}_{\texttt{SHALLOW}}$                            & 80.38    & 85.1         & 77.8    & 97.9           & 86.4          & 54.7          & 69.00   & 77.20       & 29.65      \\ 
Deep-$\mathrm{share}_{\texttt{DEEP}}$                                  & \textbf{88.28}    & \textbf{87.8}         & \textbf{84.5}    & 98.2           & \textbf{91.6}          & \textbf{79.3}          & \textbf{77.06}   & \textbf{82.28}       & \textbf{52.00}      \\
No-$\mathrm{share}_{\texttt{DEEP}}$                                    & 82.32    & 85.9         & 79.0    & 97.9           & 86.3          & 62.5          & 70.29   & 80.20       & 37.69      \\
\bottomrule
\end{tabular}}
\end{center}
\end{table}






==> arxiv/vtab_per_task.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{Per-task fine-tuning results for VTAB-1k benchmarks. We report the average accuracy over five independent runs. Best results among all methods except Finetune are \textbf{bolded}.}
\label{table:vtab}
\begin{center}
\scalebox{0.625}{
\begin{tabular}{@{}l|ccccccc|cccc|cccccccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{7}{c|}{\textbf{Natural}}                                                                         & \multicolumn{4}{c|}{\textbf{Specialized}}                      & \multicolumn{8}{c}{\textbf{Structured}}                                                                                         \\
\multicolumn{1}{c|}{}                                 & \rotatebox{90}{CIFAR-100}     & \rotatebox{90}{Caltech101}    & \rotatebox{90}{DTD }          & \rotatebox{90}{Flowers102}    & \rotatebox{90}{Pets}          & \rotatebox{90}{SVHN}          & \rotatebox{90}{Sun397}        & \rotatebox{90}{Patch Camelyon} & \rotatebox{90}{EuroSAT}       & \rotatebox{90}{Resisc45}      & \rotatebox{90}{Retinopathy}   & \rotatebox{90}{Clevr/count}   & \rotatebox{90}{Clevr/distance} & \rotatebox{90}{DMLab}         & \rotatebox{90}{KITTI/distance} & \rotatebox{90}{dSprites/loc}  & \rotatebox{90}{dSprites/ori}  & \rotatebox{90}{SmallNORB/azi} & \rotatebox{90}{SmallNORB/ele} \\ \midrule
Finetune                                              & 68.9          & 87.7          & 64.3          & 97.2          & 86.9          & 87.4          & 38.8          & 79.7           & 95.7          & 84.2          & 73.9          & 56.3          & 58.6           & 41.7          & 65.5           & 57.5          & 46.7          & 25.7          & 29.1          \\
Deep-$\mathrm{share}_{\texttt{SHALLOW}}$                                           & \textbf{76.8} & 88.9          & 62.4          & \textbf{97.7} & \textbf{86.2} & 68.0          & \textbf{50.5} & 78.6           & 90.7          & 75.7          & 73.7          & 39.2          & 55.2           & 35.4          & 55.5           & 47.7          & 35.8          & 15.0          & 24.4          \\
No-$\mathrm{share}_{\texttt{SHALLOW}}$                                            & 63.5          & 87.3          & 62.3          & 96.7          & 85.8          & 36.0          & 51.4          & 78.7           & 90.5          & 71.1          & 72.9          & 36.8          & 43.8           & 34.6          & 54.0           & 13.4          & 22.6          & 10.5          & 21.5          \\ 
Deep-$\mathrm{share}_{\texttt{DEEP}}$                                           & 75.5          & \textbf{90.7} & \textbf{65.4} & 96.6          & 86.0          & \textbf{78.5} & 46.7          & \textbf{79.5}  & \textbf{95.1} & \textbf{80.6} & \textbf{74.0} & \textbf{69.9} & \textbf{58.2}  & \textbf{40.9} & \textbf{69.5}  & \textbf{72.4} & \textbf{46.8} & \textbf{23.9} & \textbf{34.4} \\
No-$\mathrm{share}_{\texttt{DEEP}}$                                              & 70.0          & 88.5          & 62.2          & 96.7          & 85.3          & 43.5          & 45.8          & 78.0           & 93.4          & 75.7          & 73.9          & 41.5          & 55.0           & 34.1          & 60.0           & 39.6          & 31.9          & 15.4          & 24.0          \\
\bottomrule
\end{tabular}}
\end{center}
\end{table}





==> tables/hyper.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{Evaluation metrics for each dataset.}
\begin{center}
\scalebox{1.0}{
\begin{tabular}{@{}l|cccc|cccc@{}}
\toprule
\multirow{2}{*}{Datasets} & \multicolumn{4}{c|}{Deep-share} & \multicolumn{4}{c}{No-share} \\
                          & BS    & Length  & LR    & WD    & BS   & Length  & LR   & WD   \\ \midrule
CUB-200-2011              & 64    & 10      & 25.0  & 1e-4  & 64   & 10      & 50.0 & 1e-4 \\
NABirds                   & 64    & 50      & 10.0  & 1e-4  & 64   & 50      & 50.0 & 1e-4 \\
OxfordFlowers             & 64    & 5       & 10.0  & 1e-3  & 64   & 5       & 10.0 & 0    \\
StanfordDogs              & 64    & 100     & 1.0   & 1e-3  & 64   & 100     & 50.0 & 0    \\
StanfordCars              & 64    & 200     & 10.0  & 1e-4  & 64   & 200     & 50   & 0    \\ \midrule
CIFAR-100                 & 128   & 10      & 5.0   & 1e-3  & 128  & 10      & 25.0 & 1e-3 \\
Caltech101                & 128   & 10      & 5.0   & 1e-3  & 128  & 10      & 25.0 & 1e-4 \\
DTD                       & 128   & 10      & 10.0  & 1e-3  & 128  & 10      & 2.5  & 0    \\
Flowers102                & 128   & 1       & 1e-1  & 1e-3  & 128  & 1       & 1e-1 & 1e-3 \\
Pets                      & 128   & 1       & 2.5   & 1e-4  & 128  & 1       & 1.0  & 1e-4 \\
SVHN                      & 128   & 50      & 2.5   & 1e-2  & 128  & 50      & 25.0 & 1e-4 \\
Sun397                    & 128   & 5       & 1e-1  & 0     & 128  & 5       & 1e-1 & 1e-4 \\
Patch Camelyon            & 128   & 100     & 5e-1  & 1e-4  & 128  & 100     & 5.0  & 1e-4 \\
EuroSAT                   & 128   & 100     & 5.0   & 1e-3  & 128  & 100     & 50.0 & 0    \\
Resisc45                  & 128   & 10      & 10.0  & 1e-3  & 128  & 10      & 50   & 1e-4 \\
Retinopathy               & 128   & 1       & 5.0   & 1e-2  & 128  & 1       & 1e-1 & 1e-2 \\
Clevr/count               & 128   & 50      & 5.0   & 0     & 128  & 50      & 5.0  & 1e-4 \\
Clevr/distance            & 128   & 200     & 1.0   & 1e-4  & 128  & 200     & 25.0 & 0    \\
DMLab                     & 128   & 100     & 2.5   & 1e-4  & 128  & 100     & 0.25 & 1e-2 \\
KITTI/distance            & 128   & 50      & 5.0   & 0     & 128  & 50      & 0.25 & 1e-3 \\
dSprites/loc              & 128   & 10      & 5.0   & 0     & 128  & 10      & 5.0  & 0    \\
dSprites/ori              & 128   & 50      & 2.5   & 1e-4  & 128  & 50      & 10.0 & 1e-4 \\
SmallNORB/azi             & 128   & 200     & 10.0  & 1e-4  & 128  & 200     & 1.0  & 1e-3 \\
SmallNORB/ele             & 128   & 2       & 1.0   & 1e-4  & 128  & 2       & 10.0 & 1e-2 \\ \midrule
E2E                       & 10    & 5       & 1e-4  & 0     & 10   & 5       & 1e-2 & 0    \\
WebNLG                    & 5     & 5       & 1e-4  & 0     & 5    & 5       & 5e-2 & 0    \\
XSUM                      & 14    & 100     & 5e-5  & 0     & 14   & 100     & 5e-4 & 0    \\ \bottomrule
\end{tabular}}
\end{center}
\end{table}

